Point2Tree(P2T) -- framework for parameter tuning of semantic and instance segmentation used with mobile laser scanning data in coniferous forest

This article introduces Point2Tree, a novel framework that incorporates a three-stage process involving semantic segmentation, instance segmentation, optimization analysis of hyperparemeters importance. It introduces a comprehensive and modular approach to processing laser points clouds in Forestry. We tested it on two independent datasets. The first area was located in an actively managed boreal coniferous dominated forest in V{\aa}ler, Norway, 16 circular plots of 400 square meters were selected to cover a range of forest conditions in terms of species composition and stand density. We trained a model based on Pointnet++ architecture which achieves 0.92 F1-score in semantic segmentation. As a second step in our pipeline we used graph-based approach for instance segmentation which reached F1-score approx. 0.6. The optimization allowed to further boost the performance of the pipeline by approx. 4 \% points.

==> quality_measures/accuracy.tex <==
\begin{equation}
    \mathrm{accuracy} = \frac{1}{N} \sum_{i=0}^{N-1} 1 \left( Y_i = \hat{Y}_i \right),
    \label{eq:class_accuracy}
\end{equation}

\noindent
where $Y_i$ and $\hat{Y}_i$ are the $i$-th sample true categories and ones predicted by the model, respectively, and $N$ is a dataset cardinality.


==> quality_measures/accuracy_anomalies.tex <==
Given the values $t$ and $f$ representing, respectively, an amount of correctly and incorrectly classified samples, the accuracy can be defined as in (\ref{eq:accuracy}):

\begin{equation}
\mathrm{accuracy} = \frac{\mathit{t}}{\mathit{t} + \mathit{f}}.
\label{eq:accuracy}
\end{equation}

==> quality_measures/f_score_clusters.tex <==
An F-measure was used as a quality metric during conducted experiments. It is calculated using two helper metrics, a recall, also called sensitivity, and a precision. Given class $i$ and cluster $j$ those metrics are calculated as follows:

\begin{equation}
    \mathrm{recall}(i, j) = \frac{n_{ij}}{n_i},
    \label{eq:recall_clustering}
\end{equation}

\begin{equation}
    \mathrm{precision}(i, j) = \frac{n_{ij}}{n_j},
    \label{eq:precision_clustering}
\end{equation}

\noindent
where $n_{ij}$ is the number of items of class $i$ that are classified as members of cluster $j$, while $n_j$ and $n_i$ are the numbers of items in cluster $j$ and class $i$, respectively.

The clusters' $\mathrm{F}_\beta$ score is given by the following formula:

\begin{equation}
    \mathrm{F}_1(i, j) = (1 + \beta^2) \cdot \frac{\mathrm{recall}(i, j) \cdot \mathrm{precision}(i, j)}{\mathrm{recall}(i, j) + \beta^2 \cdot \mathrm{precision}(i, j)},
    \label{eq:fractional_F_measure}
\end{equation}

\noindent
where $\beta$ parameter controls the recall importance in relevance to the precision. For results presented in this paper $\beta=1$ was used.

The overall quality of the classification can be obtained by taking the weighted average $\mathrm{F}_1$ scores for each class. It is given by the equation:

\begin{equation}
    \mathrm{F}_1 = \sum\limits_{i} \frac{n_i}{n}\max{\mathrm{F}_1(i, j)},
    \label{eq:overall_F_measure}
\end{equation}

where the maximum is taken over all clusters and $n$ is the number of all objects. The $\mathrm{F}_1$ score value ranges from 0 to 1, with a higher value indicating a higher clustering quality.

==> quality_measures/f_score_tfpn.tex <==
An F-measure was used as a quality metric during conducted experiments. It is calculated using two helper metrics, a recall (\ref{eq:recall}), also called sensitivity, and a precision (\ref{eq:precision}):

\begin{equation}
    \mathrm{recall} = \frac{\mathit{tp}}{\mathit{tp} + \mathit{fn}},
    \label{eq:recall}
\end{equation}
\begin{equation}
    \mathrm{precision} = \frac{\mathit{tp}}{\mathit{tp} + \mathit{fp}},
    \label{eq:precision}
\end{equation}
where:
\begin{itemize}
    \item $\mathit{tp}$ -- true positive -- item correctly classified as an anomaly,
    \item $\mathit{fp}$ -- false positive -- item incorrectly classified as an anomaly,
    \item $\mathit{fn}$ -- false negative -- item incorrectly classified as a part of normal operation.
\end{itemize} 

The $\beta$ parameter controls the recall importance in relevance to the precision when calculating an F-measure:

\begin{equation}
    \mathrm{F}_\beta = (1 + \beta^2) \cdot \frac{\mathrm{recall} \cdot \mathrm{precision}}{\mathrm{recall} + \beta^2 \cdot \mathrm{precision}}.
    \label{eq:f_measure}
\end{equation}

During the experiments two $\beta$ values were used, \num{1} and \num{2}, to show the impact of the recall on the final score.

==> quality_measures/rmse.tex <==
\begin{equation}
\mathrm{RMSE} = {\sqrt {\frac{1} {N}{\sum\limits_{i = 1}^N {\left({y}_{\mathit{r}}^{i} - y_{\mathit{p}}^{i} \right)^{2} }}}} 
  \label{eq:rmse}
\end{equation}

\begin{equation}
\mathrm{MPE} = {\frac{100 \%} {N}{\sum\limits_{i = 1}^N \frac{{{y}_{\mathit{r}}^{i} - y_{\mathit{p}}^{i}}}{{y}_{\mathit{r}}^{i}} } }
  \label{eq:mpe}
\end{equation}

\noindent
where: ${y}_{\mathit{r}}^{i}$ and $y_{\mathit{p}}^{i}$ are a voltage time series and its predicted counterpart, respectively, and $N$ is a dataset cardinality.
